Minimum $\ell_{1}$-norm interpolators: Precise asymptotics and multiple descent

An evolving line of machine learning works observe empirical evidence that suggests interpolating estimators -- the ones that achieve zero training error -- may not necessarily be harmful. This paper pursues theoretical understanding for an important type of interpolators: the minimum $\ell_{1}$-norm interpolator, which is motivated by the observation that several learning algorithms favor low $\ell_1$-norm solutions in the over-parameterized regime. Concretely, we consider the noisy sparse regression model under Gaussian design, focusing on linear sparsity and high-dimensional asymptotics (so that both the number of features and the sparsity level scale proportionally with the sample size). We observe, and provide rigorous theoretical justification for, a curious multi-descent phenomenon; that is, the generalization risk of the minimum $\ell_1$-norm interpolator undergoes multiple (and possibly more than two) phases of descent and ascent as one increases the model capacity. This phenomenon stems from the special structure of the minimum $\ell_1$-norm interpolator as well as the delicate interplay between the over-parameterized ratio and the sparsity, thus unveiling a fundamental distinction in geometry from the minimum $\ell_2$-norm interpolator. Our finding is built upon an exact characterization of the risk behavior, which is governed by a system of two non-linear equations with two unknowns.

==> sections/simulations.tex <==
\section{Simulations}
We show some simulation results here. 
% \yuting{write out the definitions here for $\zeta, \nu$?}
For notational simplicity, let us introduce parameters 
\begin{align}
\zeta \defn \alpha \tau, \qquad
\nu \defn \frac{M}{\tau}. 
\end{align}

\paragraph{Numerical solution of the fixed-point equations.} 
The numerical solution is obtained by a two-layer binary search. For example, to solve for $\zeta(\delta)$, we construct a binary search over $\zeta$ values (by keep expanding the search range if the left and right side do not have opposite sign). For each candidate value of $\zeta$, the value of $\alpha(\zeta,\delta)$ is again obtained by a binary search. The function values are calculated by CDF and PDF of standard Gaussian functions in SciPy. The results are summarized as follows:\yue{In Figure~\ref{fig:delta}, the value of $\nu$ indicates the Lasso loss; we can see that near $\delta=0$ there is a decreasing phase.}

  \begin{minipage}{\linewidth}
	\centering
	\begin{minipage}{0.48\linewidth}
		\begin{figure}[H]
			\includegraphics[width=\linewidth]{figs/delta_zeta_plot.png}
			\caption{Plot of function $\zeta(\delta)$}
		\end{figure}
	\end{minipage}
	\hspace{0.02\linewidth}
	\begin{minipage}{0.48\linewidth}
		\begin{figure}[H]
			\label{fig:delta}
			\includegraphics[width=\linewidth]{figs/delta_nu_plot.png}
			\caption{Plot of function $\nu(\delta)$. Dots for limiting values when $\delta = 0^+$.}
		\end{figure}
	\end{minipage}
	
	\begin{minipage}{0.48\linewidth}
		\begin{figure}[H]
			\includegraphics[width=\linewidth]{figs/ge_lasso_debiased.png}
			\caption{Generalization error of the de-biased Lasso when $\lambda \goto 0^+$.}
		\end{figure}
	\end{minipage}
	\hspace{0.02\linewidth}
	\begin{minipage}{0.48\linewidth}
		\begin{figure}[H]
			\includegraphics[width=\linewidth]{figs/ge_lasso.png}
			\caption{Generalization error of Lasso when $\lambda \goto 0^+$, or sparse interpolation limit. Dots for limiting values when $\delta = 0^+$.}
		\end{figure}
	\end{minipage}
\end{minipage}


\paragraph{Weak signal versus strong signal.} We plot the generalization error for two cases, the weak signal case and the strong signal case. Recall that we use $SNR = \epsilon M^2 /\sigma^2$. We fix $SNR=2$ and $SNR=0.5$ as examples of the strong signal and weak signal case, and vary the $\epsilon$ and corresponding values of $M$. The results are shown in Figure~\ref{fig:strong-signal} and Figure~\ref{fig:weak-signal}.

We can see that, given a fixed level of signal strength, the generalization error tends to have local minimums when $\epsilon$ is small.
\begin{figure}[H]
	\centering
	\includegraphics[width=0.7\linewidth]{figs/ge_lasso_2.png}
	\caption{Comparison between the $\ell_{1}$ and $\ell_2$ interpolation limit: the strong signal case.}
	\label{fig:strong-signal}
\end{figure}
\begin{figure}[H]
	\centering
	\includegraphics[width=0.7\linewidth]{figs/ge_lasso_0_5.png}
	\caption{Comparison between the $\ell_{1}$ and $\ell_2$ interpolation limit: the weak signal case.}
	\label{fig:weak-signal}
\end{figure}

\newpage
\paragraph{Non-zero penalty.} In this part, we plot the solution of fixed point equations with non-zero $\lambda$ values. We choose two cases: (A) $M=10$, $\epsilon = 0.02$, $\lambda=10^{-2}$; (B) $M=2$, $\epsilon = 0.5$, $\lambda = 10^{-2}$. Note that the SNR is the same for the two settings. The numerical solution of the fixed point equations are also obtained by binary search.
\begin{figure}[H]
	\centering
	\includegraphics[width=0.7\linewidth]{figs/lasso_sparse.png}
	\caption{Lasso with non-zero penalty: the sparse case.}
% \yuting{why when $\delta\to 0$, you do not encounter a large error? you are estimating with $0$ right?}}
	\label{fig:sparse2}
\end{figure}


\begin{figure}[H]
	\centering
	\includegraphics[width=0.7\linewidth]{figs/lasso_non_sparse.png}
	\caption{Lasso with non-zero penalty: the non-sparse case.}
	\label{fig:non-sparse}
\end{figure}
